Stable-Hair: Real-World Hair Transfer via Diffusion Model

Current hair transfer methods struggle to handle diverse and intricate hairstyles, limiting their applicability in real-world scenarios. In this paper, we propose a novel diffusion-based hair transfer framework, named \textit{Stable-Hair}, which robustly transfers a wide range of real-world hairstyles to user-provided faces for virtual hair try-on. To achieve this goal, our Stable-Hair framework is designed as a two-stage pipeline. In the first stage, we train a Bald Converter alongside stable diffusion to remove hair from the user-provided face images, resulting in bald images. In the second stage, we specifically designed a Hair Extractor and a Latent IdentityNet to transfer the target hairstyle with highly detailed and high-fidelity to the bald image. The Hair Extractor is trained to encode reference images with the desired hairstyles, while the Latent IdentityNet ensures consistency in identity and background. To minimize color deviations between source images and transfer results, we introduce a novel Latent ControlNet architecture, which functions as both the Bald Converter and Latent IdentityNet. After training on our curated triplet dataset, our method accurately transfers highly detailed and high-fidelity hairstyles to the source images. Extensive experiments demonstrate that our approach achieves state-of-the-art performance compared to existing hair transfer methods. Project page: \textcolor{red}{\url{https://xiaojiu-z.github.io/Stable-Hair.github.io/}}

==> sections_new/Reproducibility_Checklist.tex <==
\subsection{Reproducibility Checklist}
\begin{enumerate}
\item This paper:
\begin{itemize}
    \item Includes a conceptual outline and/or pseudocode description of AI methods introduced (\answerYes{Yes})
    \item  Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results (\answerYes{Yes})
    \item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper (\answerYes{Yes})
\end{itemize}
\item Does this paper make theoretical contributions? (\answerYes{Yes})
\begin{itemize}
    \item All assumptions and restrictions are stated clearly and formally. (\answerYes{Yes})
    \item All novel claims are stated formally (e.g., in theorem statements). (\answerYes{Yes})
    \item Proofs of all novel claims are included. (\answerYes{Yes})
    \item Proof sketches or intuitions are given for complex and/or novel results. (\answerYes{Yes})
    \item Appropriate citations to theoretical tools used are given. (\answerYes{Yes})
    \item All theoretical claims are demonstrated empirically to hold. (\answerYes{Yes})
    \item All experimental code used to eliminate or disprove claims is included. (\answerYes{Yes})
\end{itemize}
\item Does this paper rely on one or more datasets? (\answerYes{Yes})
\begin{itemize}
    \item A motivation is given for why the experiments are conducted on the selected datasets (\answerYes{Yes})
    
    \item All novel datasets introduced in this paper are included in a data appendix. (\answerYes{Yes})

    \item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (\answerYes{Yes})

    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. (\answerYes{Yes})

    \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. (\answerYes{Yes})

    \item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. (\answerYes{Yes})
\end{itemize}

\item Does this paper include computational experiments? (\answerYes{Yes})

\begin{itemize}
    \item Any code required for pre-processing data is included in the appendix. (\answerNo{No}).

    \item All source code required for conducting and analyzing the experiments is included in a code appendix. (\answerNo{No})

    \item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (\answerYes{Yes})

    \item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from (\answerYes{Yes})

    \item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. (\answerYes{Yes})

    \item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. (\answerYes{Yes})

    \item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. (\answerYes{Yes})

    \item This paper states the number of algorithm runs used to compute each reported result. (\answerYes{Yes})

    \item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. (\answerYes{Yes})

    \item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). (\answerYes{Yes})

    \item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. (\answerYes{Yes})

    \item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. (\answerYes{Yes})

\end{itemize}
\end{enumerate}
